GeNAS: Neural Architecture Search with Better Generalization

Neural Architecture Search (NAS) aims to automatically excavate the optimal network architecture with superior test performance. Recent neural architecture search (NAS) approaches rely on validation loss or accuracy to find the superior network for the target data. In this paper, we investigate a new neural architecture search measure for excavating architectures with better generalization. We demonstrate that the flatness of the loss surface can be a promising proxy for predicting the generalization capability of neural network architectures. We evaluate our proposed method on various search spaces, showing similar or even better performance compared to the state-of-the-art NAS methods. Notably, the resultant architecture found by flatness measure generalizes robustly to various shifts in data distribution (e.g. ImageNet-V2,-A,-O), as well as various tasks such as object detection and semantic segmentation. Code is available at https://github.com/clovaai/GeNAS.

==> manuscripts/0_abstract_camready.tex <==
\begin{abstract}
    \jhcvpr{
    Neural Architecture Search (NAS) aims to automatically excavate the optimal network architecture with superior test performance. Recent neural architecture search (NAS) approaches rely on validation loss or accuracy to find the superior network for the target data.
   In this paper, we investigate a new neural architecture search measure for excavating architectures with better generalization.}
   We demonstrate that the flatness of the loss surface can be a promising proxy for predicting the generalization capability of neural network architectures.
   We evaluate our proposed method on various search spaces, showing similar or even better performance compared to the state-of-the-art NAS methods. \jhcvpr{Notably, the resultant architecture found by flatness measure generalizes robustly to various shifts in data distribution (e.g. ImageNet-V2,-A,-O), as well as various tasks such as object detection and semantic segmentation.} \cam{Code is available at \url{https://github.com/clovaai/GeNAS}.}
   \cam{\footnote{Full version of the paper (including the appendix) is available at \url{https://arxiv.org/abs/2305.08611}.}}
\end{abstract}

==> manuscripts/acknowledgement.tex <==
\section*{Acknowledgments}
This work was supported by the Engineering Research Center Program through the National Research Foundation of Korea (NRF) funded by the Korean Government MSIT (NRF-2018R1A5A1059921) and Institute of Information \& communications Technology Planning \& Evaluation (IITP) grant funded by the Korea government (MSIT) (No.2019-0-00075, Artificial Intelligence Graduate School Program (KAIST)).

==> tables/cifar100_transfer.tex <==
\begin{table*}[t]

\centering
\smallskip\noindent
\resizebox{0.75\linewidth}{!}{
\begin{tabular}{c||c|c|c|c}
\hline
\camtwo{Search} Metric & Params (M) & FLOPs (G) & Top-1 Acc (\%) & Top-5 Acc (\%) \\ \hline  \hline
% \cline{2-5}\
 Angle & 5.4 & 0.61 & 75.00 & 92.31 \\ \hline
 Accuracy & 5.4 & 0.60 & 75.37 & 92.23 \\ \hline
 \textbf{Flatness} & \textbf{5.2} & \textbf{0.58} & \textbf{76.05} & \textbf{92.64} \\ \hline
 Angle + Flatness & 5.4 \textcolor{blue}{(+0.0)} & 0.60 \textcolor{blue}{(-0.01)}& 75.72 \textcolor{blue}{(+0.72)}& 92.46 \textcolor{blue}{(+0.15)}\\ \hline
 Accuracy + Flatness & 5.4 \textcolor{blue}{(+0.0)} & 0.60 \textcolor{blue}{(+0.00)}& 75.85 \textcolor{blue}{(+0.48)}& 92.74 \textcolor{blue}{(+0.51)}\\ \hline
 
\end{tabular}
}
% \vspace{3mm}
\caption{Transferability of various \camtwo{search} metrics from CIFAR-100 onto ImageNet. \jh{The quantities in the parentheses denote the amount of change induced by the integrated metric from the baseline metric.} \jhtwo{Improvements from integrating $Flatness$ term is denoted with blue color.}}
\label{table:cifar100_transfer}
% \vspace{-5mm}
\end{table*}

==> tables/nas_bench_201_angle_acc_sharpness.tex <==

\begin{table}[t]
% \tiny
\centering
\tabcolsep=0.18cm % original: 0.15
\resizebox{1\linewidth}{!}{%
\begin{tabular}{@{}c|cccccc@{}}
\toprule
 
 & $\mu = 0$ & $\mu = 0.05$ & $\mu = 0.1$ & $\mu = 0.2$ & $\mu = 0.5$ & $\mu = 1$ \\ \midrule
\begin{tabular}[c]{@{}c@{}} Kendall's Tau \\(CIFAR-10)\end{tabular} & 0.7539 & 0.7531 & 0.7180 &  0.6539 & 0.5592 & 0.5262 \\ 
\bottomrule
\end{tabular}
}
% \vspace{3mm}
\caption{Kendall's Tau trend on CIFAR-10 for the $Angle+Accuracy+Sharpness$ combination \yj{to investigate the impact of the inherent flatness characteristic of accuracy-based search}. $\mu$ denotes the balancing coefficient for the sharpness term (i.e., the negation of the flatness metric), where $\mu=0$ denotes $Angle+Accuracy$ case. \yj{The result shows that sharpening (unflattening) the loss surface harms Kendall's Tau.}}
\label{table:nas_bench_201_correlation_standalone_angle_acc_sharpness}
% \vspace{-7mm}
\end{table}



==> tables/nas_bench_201_standalone.tex <==

\begin{table}[t!]

\centering
\smallskip\noindent
\resizebox{1\linewidth}{!}{
\begin{tabular}{c||c|c|c}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Searching Metric\end{tabular}} & \multicolumn{3}{c}{Kendall's Tau} \\
\cline{2-4}\
 & CIFAR-10 & CIFAR-100 & ImageNet16-120 \\ \hline \hline
 Angle  & 0.6671 & 0.6942 & 0.6342\\ \hline
 Accuracy  & 0.5701 & 0.5394 & 0.5411 \\ \hline
 Flatness & 0.6047 & 0.5918 & 0.5800 \\ \hline
 Angle + Accuracy & 0.7539 \textcolor{black}{(+0.0868)} & 0.7004 \textcolor{black}{(+0.0062)} & 0.6895 \textcolor{black}{(+0.0553)}\\ \hline
 Angle + Flatness & 0.7636 \textcolor{blue}{(+0.0965)}& 0.7619 \textcolor{blue}{(+0.0677)}& 0.7368 \textcolor{blue}{(+0.1026)}\\ \hline
 Accuracy + Flatness & 0.6023 \textcolor{blue}{(+0.0322)} & 0.5658 \textcolor{blue}{(+0.0264)} & 0.5657 \textcolor{blue}{(+0.0246)}\\ \hline
\end{tabular}
}
% \vspace{3mm}
\caption{Kendall's Tau of various \camtwo{search} proxy metrics on NAS-Bench-201. The quantities in \yj{the parentheses denote the amount of Kendall's Tau changed by the integrated metric from the baseline metric.} \jhtwo{Improvements from integrating \textit{Flatness} term is denoted with blue color.}}
\label{table:nas_bench_201_correlation_standalone_combined}
% \vspace{-7mm}
\end{table}
